FED-$\chi^2$: Privacy Preserving Federated Correlation Test

In this paper, we propose the first secure federated $\chi^2$-test protocol Fed-$\chi^2$. To minimize both the privacy leakage and the communication cost, we recast $\chi^2$-test to the second moment estimation problem and thus can take advantage of stable projection to encode the local information in a short vector. As such encodings can be aggregated with only summation, secure aggregation can be naturally applied to hide the individual updates. We formally prove the security guarantee of Fed-$\chi^2$ that the joint distribution is hidden in a subspace with exponential possible distributions. Our evaluation results show that Fed-$\chi^2$ achieves negligible accuracy drops with small client-side computation overhead. In several real-world case studies, the performance of Fed-$\chi^2$ is comparable to the centralized $\chi^2$-test.

==> figs/bimodal.tex <==
\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}
\begin{tikzpicture}
\begin{axis}[
  no markers, domain=-32:32, samples=100,
  axis lines*=left, 
  % xlabel=$x$, ylabel=$y$,
  every axis y label/.style={at=(current axis.above origin),anchor=south},
  every axis x label/.style={at=(current axis.right of origin),anchor=west},
  % height=5cm, width=12cm,
  xtick=\empty, ytick=\empty,
  enlargelimits=false, clip=false, axis on top,
  grid = major
  ]
  % \addplot [fill=cyan!20, draw=none, domain=0:5.16] {gauss(1,1)} \closedcycle;
  \addplot [very thick,cyan!50!black,domain=-32:0] {gauss(-16,4)};
  \addplot [very thick,cyan!50!black,domain=0:32] {gauss(16,4)};

  \draw [yshift=-0.6cm, latex-latex](axis cs:4,0) -- node [fill=white] {$1.96\sigma$} (axis cs:5.96,0);
\end{axis}

\end{tikzpicture}

==> prelim.tex <==
\section{Background and Notation}





\todo{make clear the contribution; stable projection is already used in frequency moments estimation;}
%
\subsection{Stable Distribution}

Stable distribution~\cite{li2009compressed} is the main building block of our protocol.
%
% a streaming algorithm for frequency moments estimation.
% %
% It projects the inputs into a random variable that follows some kind of stable distributions.
% %
% The scale of the random variable reflects the frequency moments.

\begin{definition}[$\alpha$-stable distribution]
A random variable $X$ follows an $\alpha$-stable distribution $\mathcal{Q}_{\alpha, \beta, F}$ if its characteristic function is as follow.
$$
\phi_X(t) = \exp(-F|t|^p(1-\sqrt{-1}\beta\sgn(t)\tan(\frac{\pi\alpha}{2})))
$$
, where $F$ is the scale to the $\alpha^{th}$ power and $\beta$ is the skewness.
\end{definition}

In this paper, we focus on a special subset of stable distributions, namely \emph{symmetric stable distributions} whose skewness $\beta=0$.
%
Hence, we omit the $\beta$ in the subscript and denote the distribution by $\mathcal{Q}_{\alpha, F}$.

$\alpha$-stable distribution is named due to its property called $\alpha$-stability.
%
Briefly, the sum of independent $\alpha$-stable variables still follows a $\alpha$-stable distribution with different scale.
%
\begin{definition}[$\alpha$-stability]
If random variables $X\sim\mathcal{Q}_{\alpha, 1}, Y\sim\mathcal{Q}_{\alpha, 1}$ and $X$ and $Y$ are independent, then $C_1X+C_2Y\sim\mathcal{Q}_{\alpha, C_1^\alpha+C_2^\alpha}$.
\end{definition}
